MetaSumPerceiver: Multimodal Multi-Document Evidence Summarization for Fact-Checking

Fact-checking real-world claims often requires reviewing multiple multimodal documents to assess a claim's truthfulness, which is a highly laborious and time-consuming task. In this paper, we present a summarization model designed to generate claim-specific summaries useful for fact-checking from multimodal, multi-document datasets. The model takes inputs in the form of documents, images, and a claim, with the objective of assisting in fact-checking tasks. We introduce a dynamic perceiver-based model that can handle inputs from multiple modalities of arbitrary lengths. To train our model, we leverage a novel reinforcement learning-based entailment objective to generate summaries that provide evidence distinguishing between different truthfulness labels. To assess the efficacy of our approach, we conduct experiments on both an existing benchmark and a new dataset of multi-document claims that we contribute. Our approach outperforms the SOTA approach by 4.6% in the claim verification task on the MOCHEG dataset and demonstrates strong performance on our new Multi-News-Fact-Checking dataset.

==> tmp.tex <==
\begin{table*}[!th]
\centering
\caption{Performance of claim verification in Multi-News-Fact-Checking dataset. We compare our method with Llama 2, and other offline summarization models.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccccccc}\hline
\textbf{Setting}      & \textbf{Accuracy (\%)} & \textbf{\begin{tabular}[c]{@{}c@{}}Precision (\%)\\ Entailment \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Precision (\%)\\ Contradiction\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Precision (\%)\\ Neutral\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Recall (\%)\\ Entailment\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Recall (\%)\\ Contradiction\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Recall (\%)\\ Neutral\end{tabular}} \\
\hline
PEGASUS $\rightarrow$ DeBERTAV3 & 33.2 & 64.2& 14.7& 21.5& 37.3& 12.4& 11.9 \\
PEGASUS $\rightarrow$ Llama 2 & 39.5 & 37.4& 23.1& 42.8& 27.6& 24.3& 24.0\\\hline 
T5 large $\rightarrow$ DeBERTAV3 & 34.8 & 62.8& 17.5& 26.2& 33.0& 18.5& 18.2\\
T5 large $\rightarrow$ Llama 2 & 37.2 & 40.2& 32.8& \textbf{48.0}& 30.5& 26.4& 26.8\\\hline  
PRIMERA $\rightarrow$ DeBERTAV3 & 35.9 & 68.2 & 32.7 & 23.7 & 35.8 & 23.8 & 45.1 \\
PRIMERA $\rightarrow$ Llama 2 & 39.2 & 43.5 & 47.2 & 33.1 & 47.2 & 35.5 & 24.9 \\ \hline
MSP(Entailment, LM critics) $\rightarrow$ DeBERTAV3 & 36.9 & \textbf{74.3} & 29.3 & 28.3 & 42.5 & 23.9 & \textbf{44.8}\\ 
MSP(Entailment critic) $\rightarrow$ Llama 2 & 42.6 & 41.0 & \textbf{53.7} & 34.6 & 54.8 & 37.8 & 29.6 \\
MSP(Entailment, LM critics) $\rightarrow$ Llama 2 & \textbf{46.0} & 49.5 & 49.3 & 34.1 & \textbf{56.4} & \textbf{44.7} & 28.9 \\ \hline
\end{tabular}}
\label{label:multi-news}
\end{table*}

\begin{table}[!th]\footnotesize
\centering
\caption{Performance of claim verification in MOCHEG. DeBERTaV3 and Llama 2 represent the fixed entailment models. "Gold Evidence" denotes ground truth text and image evidence, while "System Evidence" refers to automatically retrieved text and image evidence. "Human" indicates human evaluation.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c}
\hline
\textbf{Setting}                       & \textbf{F-score (\%)} \\ \hline
MSP(Entailment critic) w/ Text Evidence $\rightarrow$ DeBERTAV3           & 42.7                   \\
MSP(Entailment critic) w/ Text and Image Evidence $\rightarrow$ DeBERTAV3 & 45.1                   \\
MSP(Entailment critic) w/ Text Evidence $\rightarrow$ Llama 2           & 43.9                 \\
MSP(Entailment critic) w/ Text and Image Evidence $\rightarrow$ Llama 2 & \textbf{48.2}                   \\ \hline

MSP(Entailment, LM critics) w/ Text Evidence $\rightarrow$ DeBERTAV3           & 44.1                  \\
MSP(Entailment, LM critics) w/ Text and Image Evidence $\rightarrow$ DeBERTAV3 & 46.1                   \\
MSP(Entailment, LM critics) w/ Text Evidence $\rightarrow$ Llama 2           & 44.6                \\
MSP(Entailment, LM critics) w/ Text and Image Evidence $\rightarrow$ Llama 2 & \textbf{48.6}                   \\ \hline

MOCHEG w/ Text Evidence                 & 42.7                \\
MOCHEG w/ Image Evidence                & 40.9                \\
MOCHEG w/ Text and Image Evidence       & \textbf{44.0}                \\ \hline

Human w/o Evidence                      & 20.0                \\
Human w/ System Evidence                & 62.0                \\
Human w/ Gold Evidence                  & \textbf{70.0}                \\ \hline
\end{tabular}
}
\label{label:claim_verification_fscore_MOCHEG}
\end{table}

\begin{table}[ht]\footnotesize
\centering
\caption{Performance of claim verification in Multi-News-Fact-Checking dataset. DeBERTAV3 and Llama 2 serve as the fixed entailment models. "Gold Evidence" denotes ground truth text and image evidence, while "System Evidence" refers to automatically retrieved text and image evidence. "Human" indicates human evaluation.} 
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c}
\hline
\textbf{Setting}             & \textbf{F-score (\%)} \\\hline
PEGASUS $\rightarrow$ DeBERTAV3           & 25.4                 \\
PEGASUS $\rightarrow$ Llama 2           & \textbf{30.8}            \\\hline 
T5 large $\rightarrow$ DeBERTAV3          & 28.5            \\
T5 large $\rightarrow$ Llama 2          & \textbf{32.7}            \\\hline 
PRIMERA $\rightarrow$ DeBERTAV3 & 38.2\\
PRIMERA $\rightarrow$ Llama 2   & \textbf{38.3} \\\hline 
MSP(Entailment, LM critics) $\rightarrow$ DeBERTAV3               & 40.1            \\
MSP(Entailment critic) $\rightarrow$ Llama 2               & 41.8                 \\
MSP(Entailment, LM critics) $\rightarrow$ Llama 2               & \textbf{43.7}        \\\hline
Human w/o Evidence           & 23.0            \\
Human w/ System Evidence     & 65.0               \\
Human w/ Gold Evidence       & \textbf{76.0}               \\ \hline
\end{tabular}}
\label{label:multi-news_fscore}
\end{table}
